Language Models as Science Tutors

NLP has recently made exciting progress toward training language models (LMs) with strong scientific problem-solving skills. However, model development has not focused on real-life use-cases of LMs for science, including applications in education that require processing long scientific documents. To address this, we introduce TutorEval and TutorChat. TutorEval is a diverse question-answering benchmark consisting of questions about long chapters from STEM textbooks, written by experts. TutorEval helps measure real-life usability of LMs as scientific assistants, and it is the first benchmark combining long contexts, free-form generation, and multi-disciplinary scientific knowledge. Moreover, we show that fine-tuning base models with existing dialogue datasets leads to poor performance on TutorEval. Therefore, we create TutorChat, a dataset of 80,000 long synthetic dialogues about textbooks. We use TutorChat to fine-tune Llemma models with 7B and 34B parameters. These LM tutors specialized in math have a 32K-token context window, and they excel at TutorEval while performing strongly on GSM8K and MATH. Our datasets build on open-source materials, and we release our models, data, and evaluations.

==> tables/analysis_by_fields_complete.tex <==

\begin{table*}[ht]
\centering
\begin{tabular}{ l c c c c c}
\textbf{Models} & \textbf{Math} & \textbf{Physics} & \textbf{CS} & \textbf{Life Sci} & \textbf{Env Sci} \\ \hline
GPT-4 & 88.1 / 83.4 & 89.8 / 84.0 & 91.1 / 88.9 & 92.5 / 91.3 & 91.2 / 86.5 \\
GPT-3.5 & 72.1 / 63.4 & 73.6 / 65.9 & 79.4 / 77.1 & 80.8 / 79.6 & 79.6 / 75.8 \\ 
Zephyr-7B & 48.9 / 36.7 & 55.8 / 43.9 & 64.4 / 60.5 & 60.0 / 53.8 & 66.7 / 59.1 \\ 
Mistral-7B-v0.1 & 32.8 / 21.6 & 41.6 / 27.3 & 49.8 / 45.9 & 40.8 / 37.9 & 52.5 / 43.4 \\ 
Mistral-7B-v0.2 & 54.4 / 43.3 & 60.5 / 51.1 & 65.9 / 60.7 & 62.5 / 53.3 & 72.0 / 61.6 \\ 
Mixtral-8x7B & 65.5 / 61.8 & 68.1 / 63.1 & 75.1 / 75.0 & 73.8 / 72.9 &  78.3 / 74.2 \\ 
Vicuna-13B-16K & 37.9 / 25.6 & 41.8 / 28.5 & 55.9 / 47.2 & 56.3 / 46.3 & 48.7 / 36.8 \\ 
Tulu-2-7B & 20.2 / 12.4 & 35.5 / 22.1 & 49.2 / 32.0 & 38.9 / 27.8 & 36.2 / 29.6 \\ 
Llemma-7B-32K-Instruct & 58.8 / 45.7 & 62.4 / 51.1 & 67.5 / 56.8 & 68.3 / 55.0 & 67.3 / 53.1 \\ 
Llemma-34B-Instruct & 63.3 / 52.2 & 67.3 / 58.8 & 70.8 / 65.2 & 66.3 / 55.4 & 69.5 / 56.9 \\ 
Llemma-7B-Instruct & 57.4 / 42.9 & 60.8 / 45.3 & 64.6 / 55.0 & 58.8 / 42.5 & 57.6 / 44.3 \\ 
Llemma-7B-32K-Ultrachat & 43.7 / 34.3 & 44.8 / 37.4 & 51.7 / 50.8 & 45.0 / 41.3 & 50.9 / 43.1 \\ 
Llemma-7B-32K-ScienceChat & 57.6 / 43.2 & 62.5 / 48.6 & 63.3 / 55.0 & 64.2 / 49.2 & 61.0 / 48.4 \\
Llemma-7B-32K-MetaMath & 22.8 / 14.4 & 21.1 / 14.0 & 21.4 / 17.8 & 13.3 / ~~9.2 & 11.0 / ~~7.6 \\ 
CodeLLama-32K-MathInstruct & 54.1 / 38.4 & 56.0 / 38.6 & 65.3 / 56.3 & 
 64.2 / 42.1 & 61.0 / 41.2 \\ 
LLama-32K-MathInstruct & 33.7 / 21.0 & 45.3 / 33.9 & 53.3 / 40.0 & 67.1 / 53.8 & 39.9 / 34.3 \\
Llemma-7B-32K-MetaMath-Ultrachat & 36.5 / 29.8 & 39.4 / 29.9 & 53.4 / 47.9 & 36.3 / 32.1 & 51.3 / 39.6 \\



\end{tabular}

\caption{\howard{Table for performance by field.}}
\label{tab:analysis_by_fields_complete}
\end{table*}
